The Ultimate Combo: Boosting Adversarial Example Transferability by Composing Data Augmentations

To help adversarial examples generalize from surrogate machine-learning (ML) models to targets, certain transferability-based black-box evasion attacks incorporate data augmentations (e.g., random resizing). Yet, prior work has explored limited augmentations and their composition. To fill the gap, we systematically studied how data augmentation affects transferability. Specifically, we explored 46 augmentation techniques originally proposed to help ML models generalize to unseen benign samples, and assessed how they impact transferability, when applied individually or composed. Performing exhaustive search on a small subset of augmentation techniques and genetic search on all techniques, we identified augmentation combinations that help promote transferability. Extensive experiments with the ImageNet and CIFAR-10 datasets and 18 models showed that simple color-space augmentations (e.g., color to greyscale) attain high transferability when combined with standard augmentations. Furthermore, we discovered that composing augmentations impacts transferability mostly monotonically (i.e., more augmentations $\rightarrow$ $\ge$transferability). We also found that the best composition significantly outperformed the state of the art (e.g., 91.8% vs. $\le$82.5% average transferability to adversarially trained targets on ImageNet). Lastly, our theoretical analysis, backed by empirical evidence, intuitively explains why certain augmentations promote transferability.

==> adv-surrogates.tex <==
\section{Transferability of Adversarially Trained Surrogates}

\subsection{Methodology}

\subsection{Results}

%


==> app-alter-epsilon.tex <==
\section{The other results with various epsilons}

\begin{table*}[htbp]
\small
\centering
\caption{\label{tab:app:imageneteps}Transferability rates (\%)
  from normally trained surrogates (rows) to normally
  target models (columns) using different  $\epsilon$ on Imagenet} 
\begin{tabular}{l | l | r r r r r r r r r r r r}
\toprule

  \textbf{Epsilon} & \textbf{Attack}& \textbf{Inc-v3}& \textbf{Inc-v4}&\textbf{Res-152}&\textbf{IncRes-v2}&\textbf{ Res-50}&\textbf{ Res-101}\\ \midrule
  \multirow{5}{*}{8/255}&\ASDTM{}&98.7&75.0&60.6&69.3&68.3&62.7\\
     &\SDTM{}&99.7&77.1&62.9&70.9&69.8&64.8\\
     &\sdtv{}&99.5&77.9&64.1&72.9&72.2&66.7\\

& \gsdt{}&\textit{99.5}&\textit{81.3}&\textit{71.1}&\textit{77.6}&\textit{77.3}&\textit{72.0}\\


 & \bestcombo{}&\textbf{99.7}&\textbf{86.0}&\textbf{75.0}&\textbf{81.8}&\textbf{81.2}&\textbf{76.3}\\
 
  \hline 
   \multirow{5}{*}{24/255}&\ASDTM{}&99.9&97.1&93.7&95.9&94.8&94.4\\
     &\SDTM{}&100.0&97.8&93.6&96.8&95.1&93.9\\
     &\sdtv{}&100.0&97.9&95.0&97.1&96.2&95.6\\
& \gsdt{}&\textit{100.0}&\textit{98.5}&\textit{96.7}&\textit{98.7}&\textit{97.0}&\textit{97.0}\\


 & \bestcombo{}&\textbf{100.0}&\textbf{99.3}&\textbf{97.4}&\textbf{99.2}&\textbf{97.5}&\textbf{98.4}\\




\bottomrule
\end{tabular}


\end{table*}


==> app-cifar-aug.tex <==

\begin{table*}[!t]
\scriptsize
\caption{\label{tab:traugs}Transferability experiments on \cifarten{} using varied 
augmentations in the attacks and in the training process of the surrogate and target models. The 
experiments include Inception (I) and ResNet-50 (R) architectures, each trained without 
augmentations (i.e., Vanilla), or with horizontal flipping (HF), random cropping (RC), or 
both. The attacks used \mifgsm (MI), or \mifgsm{} augmented with HF, RC, or both.
Attacks within the same architecture when the training augmentations of the surrogate and
target are identical were performed between models trained with different initializations.}
 \centerline{
\begin{tabular}{@{}l@{\hskip.3cm}l @{\hskip.3cm}| r@{\hskip.3cm}r@{\hskip.3cm}r@{\hskip.3cm}r | r@{\hskip.3cm}r@{\hskip.3cm}r@{\hskip.3cm}r | r@{\hskip.3cm}r@{\hskip.3cm}r@{\hskip.3cm}r | r@{\hskip.3cm}r@{\hskip.3cm}r@{\hskip.3cm}r}
  \toprule
  \multicolumn{18}{c}{Inception (I) surrogates to Inception (I) targets} \\ \hline
  &Surrogate & \multicolumn{4}{c|}{\ivanilla{}} & \multicolumn{4}{c|}{\ihf{}} & \multicolumn{4}{c|}{\irc{}} & \multicolumn{4}{c}{\iall{}} \\ 
  &Target & \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}\\ \hline
  \multirow{4}{*}{\rotatebox[origin=c]{90}{Attack}} & MI     & 92.3&80.6&82.4&78.7  &  79.3&82.9&81.4&79.9  &  82.7&82.4&85.7&83.4  &  72.9&76.8&77.7&81.9 \\
  & RC-MI  & 95.0&85.1&86.1&83.1  &  \textbf{85.1}&86.7&\textbf{86.4}&85.6  &  83.6&82.9&86.8&84.3  &  75.6&\textbf{80.0}&79.0&\textbf{83.0} \\
  & HF-MI  & 92.5&84.8&85.7&83.8  &  81.8&85.4&82.6&81.5  &  87.5&86.6&88.4&88.7  &  75.0&77.8&79.0&82.6 \\
  & Both-MI & \textbf{96.2}&\textbf{90.8}&\textbf{89.4}&\textbf{88.3}  &  84.3&\textbf{87.3}&86.2&\textbf{86.7}  &  \textbf{88.8}&\textbf{88.2}&\textbf{89.9}&\textbf{89.1}  &  \textbf{75.9}&79.7&\textbf{80.2}&\textbf{83.0} \\
  
  \midrule
  \multicolumn{18}{c}{ResNet (R) surrogates and ResNet (R) targets} \\ \hline
  & Surrogate & \multicolumn{4}{c|}{\rvanilla{}} & \multicolumn{4}{c|}{\rhf{}} & \multicolumn{4}{c|}{\rrc{}} & \multicolumn{4}{c}{\rall{}} \\ 
  & Target & \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}\\ \hline
  \multirow{4}{*}{\rotatebox[origin=c]{90}{Attack}} & MI &     91.7&89.7&78.5&79.2 & 85.5&92.3&83.4&86.4 & 59.2&68.0&82.7&79.7 & 52.0&63.5&74.2&81.7 \\
  & RC-MI &  95.8&94.7&91.7&89.7 & 92.2&96.5&92.7&95.3 & 67.4&75.5&87.3&84.8 & 57.6&74.7&82.9&87.9 \\
  & HF-MI &  93.1&92.5&84.5&84.7 & 91.4&95.9&89.5&92.7 & 67.5&76.6&86.5&86.5 & 60.0&73.3&82.7&89.3 \\
  & Both-MI & \textbf{96.4}&\textbf{95.9}&\textbf{93.3}&\textbf{91.6} & \textbf{94.7}&\textbf{97.4}&\textbf{94.0}&\textbf{96.6} & \textbf{71.8}&\textbf{79.9}&\textbf{89.5}&\textbf{88.0} & \textbf{64.8}&\textbf{76.8}&\textbf{86.0}&\textbf{89.4} \\

  \midrule
  \multicolumn{18}{c}{Inception (I) surrogates and ResNet (R) targets} \\ \hline
  & Surrogate & \multicolumn{4}{c|}{\ivanilla{}} & \multicolumn{4}{c|}{\ihf{}} & \multicolumn{4}{c|}{\irc{}} & \multicolumn{4}{c}{\iall{}} \\ 
  & Target & \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}  &  \rvanilla{}&\rhf{}&\rrc{}&\rall{}\\ \hline
  \multirow{4}{*}{\rotatebox[origin=c]{90}{Attack}} & MI     & 38.2&39.1&38.8&42.3 & 35.7&36.8&38.7&42.7 & 39.3&41.0&44.0&45.8 & 32.5&36.2&36.8&42.2 \\
  & RC-MI  & 39.6&40.9&43.2&44.6 & 37.4&39.4&38.9&43.2 & 37.8&41.2&44.5&46.1 & 34.7&\textbf{38.9}&\textbf{40.0}&44.0 \\
  & HF-MI  & 39.4&43.6&44.3&47.1 & 36.6&37.6&39.1&42.4 & 41.9&44.2&47.2&50.6 & 33.6&36.6&37.3&42.6 \\
  & Both-MI & \textbf{43.5}&\textbf{47.6}&\textbf{46.5}&\textbf{48.9} & \textbf{38.2}&\textbf{40.3}&\textbf{40.5}&\textbf{45.4} & \textbf{43.6}&\textbf{44.8}&\textbf{50.4}&\textbf{51.4} & \textbf{33.9}&37.7&38.7&\textbf{44.3} \\

  \midrule
  \multicolumn{18}{c}{ResNet (R) surrogates and Inception (I) targets} \\ \hline
  & Surrogate & \multicolumn{4}{c|}{\rvanilla{}} & \multicolumn{4}{c|}{\rhf{}} & \multicolumn{4}{c|}{\rrc{}} & \multicolumn{4}{c}{\rall{}} \\ 
  & Target & \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}  &  \ivanilla{}&\ihf{}&\irc{}&\iall{}\\ \hline
  \multirow{4}{*}{\rotatebox[origin=c]{90}{Attack}} & MI     & 80.6&77.6&76.6&71.7 & 82.4&82.7&80.4&81.6 & 72.5&71.7&72.5&72.0 & 65.8&68.0&70.0&70.3 \\
  & RC-MI  & 92.3&90.0&92.0&88.1 & 93.2&93.8&92.5&92.5 & 79.3&79.6&80.8&79.4 & 75.6&78.2&79.6&80.0 \\
  & HF-MI  & 86.6&84.7&83.9&81.4 & 89.0&90.0&88.2&87.9 & 80.3&80.9&82.7&82.3 & 74.9&78.6&79.0&79.6 \\
  & Both-MI & \textbf{94.3}&\textbf{91.6}&\textbf{93.2}&\textbf{89.2} & \textbf{95.4}&\textbf{94.9}&\textbf{94.8}&\textbf{94.8} & \textbf{82.2}&\textbf{83.4}&\textbf{85.6}&\textbf{83.6} & \textbf{79.4}&\textbf{81.8}&\textbf{83.2}&\textbf{83.7} \\

 \midrule
\bottomrule
\end{tabular}
}
\end{table*}






 






==> app-cifar.tex <==
\section{Transferability Rates on \cifarten{}}
\label{app:cifar10}

\tabref{tab:app:cifar1}
reports attack
tranferability rates from all six normally trained \dnn{}s to all
other victim \dnn{}s for $\epsilon$=0.02 and $\epsilon$=0.04,
respectively.

\begin{table*}[t!]
\scriptsize
\centering
\caption{\label{tab:app:cifar1} Average transferability rates (\%) on \cifarten{},
  from normally trained surrogates (second column) to other normally trained target models  (columns), with a perturbation norm $\epsilon$=0.02 and  0.04 .need to be updated} 
\resizebox{0.75\textwidth}{!}{\begin{tabular}{l | l |  r r r r | r r r}
\toprule
    \textbf{ $\epsilon$}  &\textbf{Surrogate}  & \textbf{\ASDTM{} }& \textbf{\SDTM{}} & \textbf{\sdtv{}} & \textbf{\undp{}} & \textbf{\gsdt{}}&\textbf{\bestcombo{}} &  \textbf{\advancedultimatecombo{}}\\
\midrule
  \multirow{7}{*}{0.02}& \textbf{VGG}&51.3&54.3&24.2&28.1&55.7&\textit{61.4}&\textbf{63.0} \\&
  \textbf{Res}&50.6&54.2&20.0&24.7&57.0&\textit{64.2}&\textbf{67.9}\\&
    \textbf{DenseNet}&46.2&49.1&19.3&21.2&52.3&\textit{60.0}&\textbf{65.2}\\&
    \textbf{MobileNet}&39.2&41.6&22.3&29.3&42.0&\textit{48.0}&\textbf{53.5}\\&
    \textbf{GoogleNet}&
    41.7&43.0&27.6&34.9&43.5 &\textit{47.4}&\textbf{54.0}\\&
    \textbf{GoogleNet}&41.7&43.0&27.6&34.9&43.5&\textit{47.4}&\textbf{54.0}\\
    &\textbf{Inc}&38.5&38.3&23.3&33.4&38.1&\textit{46.1}&\textbf{54.1}\\
   \midrule 

   \multirow{7}{*}{0.04}&
   \textbf{VGG}&82.5&85.2&55.6&68.7&85.9&\textit{90.2}&\textbf{93.3} \\
   &\textbf{Res}&83.3&84.4&45.7&61.4&86.8&\textit{91.5}&\textbf{94.8}\\
   &\textbf{DenseNet}&74.6&77.7&41.3&51.7&81.6&\textit{88.7}&\textbf{93.0}\\
   &\textbf{MobileNet}&68.8&70.8&48.3&62.1&70.7&\textit{77.8}&\textbf{82.9}\\
   &\textbf{GoogleNet}&68.2&69.7&51.9&64.5&68.5&\textit{72.8}&\textbf{81.6}\\
   &\textbf{Inc}&65.6&65.1&47.3&59.4&63.6&\textit{73.5}&\textbf{83.6}\\

\bottomrule
\end{tabular}}

\end{table*}


\begin{table*}[htbp]
\small
\centering
\caption{\label{tab:app:cifar1}Transferability rates (\%) on \cifarten{},
  from normally trained surrogates (rows) to normally trained target models
  (columns), with a perturbation norm $\epsilon$=0.02.} 
\begin{tabular}{l | l | r r r r r r| r}
\toprule

  \textbf{Model} & \textbf{Attack} & \textbf{VGG}& \textbf{Res}&\textbf{DenseNet}&\textbf{MobileNet}&\textbf{GoogleNet}&\textbf{Inc}&\textbf{Avg.}\\ \midrule
  \multirow{7}{*}{VGG}
       &\ASDTM{}&81.0&41.1&42.1&61.6&53.3&58.5&51.3\\
        &\SDTM{}&82.0&46.2&\textit{46.0}&64.1&54.2&60.8&54.3\\&
         \sdtv{}&37.6&17.7&19.2&29.1&28.4&27.8&24.4\\
         & \undp{}&37.0&22.9&23.5&33.5&30.0&30.6&28.1\\ 
&        \gsdt{}&{83.8}&{46.7}&{45.3}&{66.2}&{56.0}&{64.2}&55.7\\
 & \bestcombo{}&\textbf{86.8}&\textit{52.8}&\textit{52.9}&\textit{70.9}&\textit{60.6}&\textit{69.6}  &\textit{61.4} 
\\&
\advancedultimatecombo{}&\textit{84.1}&\textbf{54.0}&\textbf{54.7}&\textbf{72.0}&\textbf{63.8}&\textbf{70.6} &\textit{63.0} \\
 \hline 
   \multirow{7}{*}{Res}&\ASDTM{}&33.9&79.1&53.0&60.4&51.3&54.4&50.6\\

     &\SDTM{}&34.4&82.1&59.1&64.5&54.4&58.6&54.2\\&
        \sdtv{}&16.6&27.1&18.2&24.2&23.2&21.7&20.8\\
     & \undp{}&20.2&31.6&22.6&27.0&26.8&26.9&24.7\\
& \gsdt{}&{38.3}&{83.1}&{60.2}&{68.3}&{54.9}&{63.5}&57.0\\

 & \bestcombo{}&\textit{44.5}&\textit{87.3}&\textit{68.6}&\textit{74.6}&\textit{62.3}&\textit{70.9}&\textit{64.2}\\
 &\advancedultimatecombo{}&\textbf{49.9}&\textbf{87.5}&\textbf{71.1}&\textbf{77.4}&\textbf{68.4}&\textbf{72.7}&\textbf{67.9}\\
 \hline 

   \multirow{7}{*}{DenseNet}&\ASDTM{}&32.9&49.2&79.7&49.4&47.5&51.8&46.2\\
     &\SDTM{}&32.3&54.1&81.0&56.1&48.9&54.3&49.1\\&
        \sdtv{}&15.4&17.5&27.0&21.2&21.1&21.3&19.3\\
        & \undp{}&18.4&19.9&30.4&23.1&21.5&23.3&21.2\\
& \gsdt{}&{35.2}&{55.4}&{82.5}&{60.3}&{50.9}&{59.9}&52.3\\

 & \bestcombo{}&\textit{40.6}&\textit{65.7}&\textit{87.4}&\textit{67.3}&\textit{59.0}&\textit{67.4}&\textit{60.0}\\
 &\advancedultimatecombo{}&\textbf{46.9}&\textbf{66.8}&\textbf{88.3}&\textbf{71.4}&\textbf{68.4}&\textbf{72.7}&\textbf{65.2}\\
 \hline 

   \multirow{7}{*}{MobileNet}&\ASDTM{}&23.7&24.3&22.3&97.3&58.9&66.6&39.2\\

     &\SDTM{}&24.9&\textit{26.1}&\textit{24.2}&98.4&62.0&70.7&41.6\\
     &
        \sdtv{}&16.4&14.7&13.7&59.8&33.8&36.5&23.0\\ &\undp{}&20.5&18.4&18.7&73.5&41.5&47.6&29.3\\


& \gsdt{}&{25.6}&25.4&23.7&{98.6}&{62.4}&{72.7}&42.0\\

 & \bestcombo{}&\textit{29.0}&\textit{31.4}&\textit{29.9}&\textbf{99.5}&\textit{70.8}&\textit{78.5}&\textit{48.0}\\
 &\advancedultimatecombo{}&\textbf{33.0}&\textbf{37.3}&\textbf{34.6}&\textit{99.4}&\textbf{78.9}&\textbf{83.6}&\textbf{53.5}\\
 \hline 
 
    \multirow{7}{*}{GoogleNet}&\ASDTM{}&24.0&23.6&22.1&71.1&\textit{99.7}&67.6&41.7\\

     &\SDTM{}&{24.1}&25.2&24.7&{71.3}&99.6&69.6&43.0\\
     &
        \sdtv{}&8.4&18.0&15.9&49.6&73.3&43.4&29.1\\
        & \undp{}&22.0&22.1&20.7&55.9&85.9&53.9&34.9\\

& \gsdt{}&{22.9}&{26.5}&{25.6}&{71.3}&98.9&{71.1}&43.5\\

 & \bestcombo{}&\textit{24.9}&\textit{29.0}&\textit{27.9}&\textit{78.6}&\textbf{99.9}&\textit{76.6}&\textit{47.4}\\
 &\advancedultimatecombo{}&\textbf{32.7}&\textbf{35.7}&\textbf{34.0}&\textbf{85.1}&\textit{99.8}&\textbf{82.5}&\textbf{54.0}\\
 \hline 
 
    \multirow{7}{*}{Inc}&\ASDTM{}&{21.9}&22.3&{21.8}&{67.2}&{59.5}&96.9&38.5\\

     &\SDTM{}&21.4&{24.1}&{22.7}&65.8&57.3&96.5&38.3\\
          &
        \sdtv{}&15.9&16.1&13.0&41.7&35.1&58.5&24.4\\
        & \undp{}&21.9&22.6&21.2&53.8&47.6&79.4&33.4\\
& \gsdt{}&21.6&24.0&21.9&65.3&57.7&\textit{98.1}&38.1\\
 & \bestcombo{}&\textit{27.0}&\textit{30.4}&\textit{28.6}&\textit{75.7}&\textit{68.8}&\textit{99.1}&\textit{46.1}\\
 &\advancedultimatecombo{}&\textbf{31.7}&\textbf{37.0}&\textbf{37.2}&\textbf{85.4}&\textbf{79.0}&\textbf{99.5}&\textbf{54.1}\\
 


 

\bottomrule
\end{tabular}


\end{table*}


\begin{table*}[htbp]
\small
\centering
\caption{\label{tab:app:cifar2}Transferability rates (\%) on \cifarten{},
  from normally trained surrogates (rows) to normally trained target models
  (columns), with a perturbation norm $\epsilon$=0.04.}
\begin{tabular}{l | l | r r r r r r|r}
\toprule

  \textbf{Model} & \textbf{Attack} & \textbf{VGG}& \textbf{Res}&\textbf{DenseNet}&\textbf{MobileNet}&\textbf{GoogleNet}&\textbf{Inc}&\textbf{Avg. }\\ \midrule
  \multirow{7}{*}{VGG}&\ASDTM{}&96.9&76.3&78.8&89.2&78.8&89.3&82.5\\

     &\SDTM{}&{98.2}&{81.1}&{82.9}&89.3&81.7&91.2&85.2\\         &
        \sdtv{}&76.3&49.1&52.9&67.7&59.2&65.3&58.8\\& \undp{}&79.3&60.3&63.9&76.8&67.8&74.6&68.7\\
& \gsdt{}&{98.2}&80.6&82.7&91.2&{82.6}&{92.5}&85.9\\

 & \bestcombo{}&\textbf{99.3}&\textit{87.0}&\textit{87.9}&\textit{93.5}&\textit{87.3}&\textit{95.3}&\textit{90.2}\\
 &\advancedultimatecombo{}&\textit{99.1}&\textbf{91.4}&\textbf{91.6}&\textbf{96.7}&\textbf{90.8}&\textbf{95.9}&\textbf{93.3}\\
 \hline 
   \multirow{7}{*}{Res}&\ASDTM{}&68.3&97.5&89.0&88.7&82.3&88.2&83.3\\

     &\SDTM{}&71.0&97.0&90.0&89.4&81.9&89.8&84.4\\
      &\sdtv{}&34.3&60.3&48.0&55.6&47.8&53.2&47.8\\
      & \undp{}&48.6&68.2&63.6&67.1&59.7&68.2&61.4\\
& \gsdt{}&{73.6}&{98.0}&{92.6}&{90.9}&{84.9}&{92.1}&86.8\\


 & \bestcombo{}&\textit{81.9}&\textit{99.3}&\textit{95.7}&\textit{95.0}&\textit{89.5}&\textit{95.6}&\textit{91.5}\\
 &\advancedultimatecombo{}&\textbf{87.6}&\textbf{99.8}&\textbf{97.7}&\textbf{97.4}&\textbf{93.7}&\textbf{97.4}&\textbf{94.8}\\
 \hline 

   \multirow{7}{*}{DenseNet}&\ASDTM{}&61.7&79.0&94.7&78.5&72.6&81.0&74.6\\

     &\SDTM{}&62.9&83.1&96.9&81.4&75.8&85.1&77.7\\&
        \sdtv{}&32.6&42.0&57.1&47.6&46.5&52.2&44.2\\
        & \undp{}&42.8&50.2&66.8&56.7&50.9&58.0&51.7\\
& \gsdt{}&{68.0}&{86.2}&{98.1}&{85.7}&{80.3}&{88.0}&81.6\\

 & \bestcombo{}&\textit{78.0}&\textit{94.1}&\textit{99.2}&\textit{91.3}&\textit{87.1}&\textit{93.1}&\textit{88.7}\\
&\advancedultimatecombo{}&\textbf{85.6}&\textbf{96.2}&\textbf{99.4}&\textbf{95.8}&\textbf{90.4}&\textbf{96.9}&\textbf{93.0}\\
 \hline 

   \multirow{7}{*}{MobileNet}&\ASDTM{}&52.2&58.3&57.6&\textit{99.9}&83.4&92.6&68.8\\

     &\SDTM{}&53.4&{61.5}&{59.6}&{99.9}&86.1&93.5&70.8\\&
        \sdtv{}&37.2&38.1&35.1&88.0&66.8&76.1&50.7\\
        & \undp{}&48.7&48.7&50.5&96.5&77.0&85.6&62.1\\

& \gsdt{}&{53.8}&59.9&57.8&{99.9}&{87.1}&{95.0}&70.7\\


 & \bestcombo{}&\textit{62.1}&\textit{69.5}&\textit{67.8}&\textbf{100.0}&\textit{92.3}&\textit{97.2}&\textit{77.8}\\
 &\advancedultimatecombo{}&\textbf{68.5}&\textbf{77.0}&\textbf{74.8}&\textbf{100.0}&\textbf{96.0}&\textbf{98.4}&\textbf{82.9}\\
 \hline 
 
    \multirow{7}{*}{GoogleNet}&\ASDTM{}&49.5&55.3&54.6&88.6&\textbf{100.0}&{93.0}&68.2\\

     &\SDTM{}&{50.7}&{57.2}&{56.2}&{90.1}&\textbf{100.0}&{94.3}&69.7\\&
        \sdtv{}&38.7&43.1&39.8&74.3&89.2&76.2&54.4\\
        & \undp{}&47.4&53.3&53.2&83.4&96.7&85.2&64.5\\
& \gsdt{}&50.1&56.1&54.9&88.9&\textbf{100.0}&92.7&68.5\\


 & \bestcombo{}&\textit{53.6}&\textit{61.6}&\textit{61.2}&\textit{92.5}&\textbf{100.0}&\textit{95.1}&\textit{72.8}\\
 &\advancedultimatecombo{}&\textbf{65.9}&\textbf{73.1}&\textbf{73.6}&\textbf{97.6}&\textbf{100.0}&\textbf{97.8}&\textbf{81.6}\\
 \hline 
 
    \multirow{7}{*}{Inc}&\ASDTM{}&{51.2}&{55.2}&54.8&{85.2}&{81.8}&99.5&65.6\\

     &\SDTM{}&50.0&54.8&\textit{55.2}&83.9&81.5&99.5&65.1\\&
        \sdtv{}&36.3&39.1&35.9&69.6&63.5&83.2&48.9\\
        & \undp{}&48.2&49.6&49.0&75.7&74.7&90.6&59.4\\
& \gsdt{}&49.0&53.3&51.9&82.8&80.9&{99.8}&63.6\\
 & \bestcombo{}&\textit{59.0}&\textit{64.8}&\textit{65.5}&\textit{90.3}&\textit{88.1}&\textbf{100.0}&\textit{73.5}\\
 &\advancedultimatecombo{}&\textbf{70.6}&\textbf{75.6}&\textbf{78.5}&\textbf{97.1}&\textbf{96.0}&\textbf{100.0}&\textbf{83.6}\\
 
\bottomrule
\end{tabular}

\end{table*}


==> app-compositions.tex <==
\section{Parallel and Serial Compositions of Augmentations}
\label{app:compositions}

\figref{fig:compositions} illustrates how parallel and serial compositions work.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/compositions2.pdf}
    \caption{\label{fig:compositions}An illustration of serial and parallel 
    compositions. When serially composing augmentations, each augmentation method
    operates on the output of the previous one. By contrast, in parallel composition,
    each augmentation method operates independently on the input (or set of inputs).
    The number of samples grows exponentially in serial composition, whereas it
    grows linearly in parallel composition. We use serial composition when composing
    diverse inputs (DI), scaling (Sc.), and translations (Tr.). Other augmentation
    methods are composed in parallel.}
\end{figure}


==> app-defense-parameters.tex <==
\section{Defense Parameters}
\label{app:defparams}

We used standard parameters when attacking defenses. For
\randsmooth{}, we used a normally trained ResNet-50 and set $\sigma$
to 0.25, following~\cite{cohen2019certified}. For \arandsmooth{}, the
target model was ResNet-50 trained with  isotropic Gaussian-noise
augmentations (sampled from $\mathcal{N}(0,0.25)$), and $\sigma$ was
set to 0.25 during prediction, per~\cite{salman2019provably}. In both
cases, we used 10,000 noisified samples during inference.
For \bitred, we used a squeezer with bit-depth of two, in accordance
with~\cite{xu2018feature}. Finally, we used the default \nrp{}
parameters and pre-trained model from the official GitHub
repository~\cite{naseer2020self}.


==> app-gen.tex <==
\section{Comparing Exhaustive and Genetic Search on a Small Search Space}
\label{app:gen}

\tabref{tab:genetic-result} and \tabref{tab:genetic-overhead} compare
between genetic and exhaustive search performance (transferability
rates and fraction of search space covered) under different population
sizes and genetic search iterations.

\input{tables/genetic-result}
\input{tables/genetic-overhead}


==> app-individual-augs.tex <==
\section{Individual Augmentations}
\label{app:indaugs}

\tabref{tab:app:weaksingle} presents the transferability rates
when integrating individual augmentation methods into \mifgsm{}. 
Trasnferability rates were computed on \imagenet{}, using the
Inc-v3 \dnn{} as a surrogate and the other normally trained \dnn{}s
as victims ($\epsilon=\frac{16}{255}$). %


\begin{table*}[hp!]
\small
\centering
\caption{\label{tab:app:weaksingle}Transferability rates
  (\%) on \imagenet{} from a normally trained Inc-v3 surrogate to normally trained target models
  (columns) when integrating individual augmentation methods into
  \mifgsm{}-based attacks .
}
\begin{tabular}{ l | r r r r r r}
\toprule
   \textbf{Attack} & \textbf{Inc-v3}& \textbf{Inc-v4}&\textbf{Res-50}&\textbf{Res-101}&\textbf{Res-152}&\textbf{IncRes-v2}\\ \midrule
MI-FGSM& \textbf{100.0} &54.7&48.9&43.5&41.1&50.6\\
\fancyPCA{}-MI-FGSM& \textbf{100.0} &\textbf{70.7}&\textbf{65.4}&\textbf{59.6}&\textbf{57.6}&\textbf{69.2}\\
\chanshuffle{}-MI-FGSM& \textbf{100.0} &57.5&54.7&49.9&46.3&56.7\\
\colorjitter{}-MI-FGSM&\textbf{100.0}&\textit{66.4}&\textit{61.8}&\textit{57.5}&\textit{54.7}&\textit{65.4}\\
\greyscale{}-MI-FGSM&\textbf{100.0}&62.9&61.4&56.5&51.8&62.4\\
\randerase{}-MI-FGSM&\textbf{100.0}&55.1&52.1&46.6&43.9&52.2\\
\cutmix{}-MI-FGSM&63.0&34.7&33.9&30.0&33.1&31.2\\
\cutout{}-MI-FGSM&\textbf{100.0}&58.2&54.4&49.6&45.7&55.9\\
\neuraltrans{}-MI-FGSM&96.4&44.4&39.5&35.6&33.6&38.2\\
\sharpen{}-MI-FGSM
&99.3&44.7&41.0&34.3&34.4&40.2\\
\autoaug{}-MI-FGSM
&\textbf{100.0}&61.1&56.6&50.1&48.5&58.4\\

\bottomrule
\end{tabular}

\end{table*}






  







==> app-models.tex <==
\section{\dnn{}s Used in the Experiments}
\label{app:models}

We tested transferability using ten \imagenet{} \dnn{}s
and six \cifarten{} \dnn{}s.
Of the ten \imagenet{} models, six were normally
trained, while others were adversarially
trained. Specifically, for normally trained models, we selected: 
Inception-v3 (Inc-v3)~\cite{szegedy2016rethinking}; Inception-v4
(Inc-v4); Inception-ResNet-v2
(IncRes-v2)~\cite{szegedy2017inception}); ResNet-v2-50 (Res-50);
ResNet-v2-101 (Res-101); and ResNet-v2-152
(Res-152)~\cite{he2016identity}. For adversarially trained models, we
selected: Inception-v3-adv
(Inc-v3$_\mathit{adv}$)~\cite{kurakin2016adversarial};
ens3-Inception-v3 (Inc-v3$_\mathit{ens3}$); ens4-Inception-v3 
(Inc-v3$_\mathit{ens4}$); and ens-adv-Inception-ResNet-v2
(IncRes-v2$_{ens}$)~\cite{tramer2017ensemble}. 
We obtained the models' PyTorch implementations and
weights from a public GitHub
repository.\footnote{\url{https://github.com/ylhz/tf_to_pytorch_model}}
All six \cifarten{} \dnn{}s were normally
trained. For this dataset, we used pre-trained VGG-11 (VGG) ~\cite{vgg}),
ResNet-50 (Res)~\cite{he2016identity}, DenseNet-121 (DenseNet)~\cite{huang2017densely}, MobileNet-v2 (MobileNet)~\cite{sandler2018mobilenetv2},
GoogleNet~\cite{szegedy2015going}, and an Inception-v3 (Inc) \dnn{}s~\cite{szegedy2016rethinking}, also implemented in PyTorch.\footnote{\url{https://github.com/huyvnphan/PyTorch_CIFAR10}}


==> app-monotonicity.tex <==
\section{The Monotonicity of Transferability When Adding Augmentations}
\label{app:monotonic}

\figref{fig:monotonic} depicts a visual summary of the experiment
presented in \secref{sec:res:monotonic}, demonstrating how the
relationship between augmentation methods and transferability is
mostly monotonic.


\begin{sidewaysfigure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/monotonic.jpg}
    \caption{\label{fig:monotonic} Best viewed after zooming in. Each
      node represents a composition of augmentation methods. The
      binary string within a node encodes the composition:
      Each bit, from the most to the least
      significant, denotes whether \admix{} (most significant bit),
      \greyscale{}, \cutout{}, \autoaug{}, DST(the combination of DI, SI and TI), \neuraltrans{}, 
      and \sharpen{} (least significant bit), respectively, is
      included (1) or excluded (0) from the composition. An edge from
      node $u$ to $v$ is included if $v$ includes exactly one more
      augmentation method compared to $u$. As explained in
      \secref{sec:res:monotonic}, we computed the average
      transferability rate per composition on \imagenet{}, from an Inc-v3
      surrogate \dnn{} to the remaining nine models as victim
      models. An edge $(u,v)$ is colored in black (resp.\ red) if
      $v$'s composition achieves higher or equal (resp.\ lower) average
      transferability rates than $u$ when integrated into
      \mifgsm{}. We faded away nodes containing \neuraltrans{} or
      \sharpen{} and their corresponding edges. Notice how all the
      remaining (unfaded) edges are black, showing that the
      relationship between the (average) transferability and the 
      remaining augmentations is monotonic (i.e., more augmentations
      composed $\rightarrow$ $\ge$transferability). Said differently,
      only \neuraltrans{} and \sharpen{} harm transferability in some
      cases.}
\end{sidewaysfigure*}


==> app-other-attacks.tex <==
\section{Attacks Considered but Excluded}
\label{app:otherattacks}

Besides the three state-of-the-art baselines we experimented with, 
we considered including two other attacks in the evaluation. (\cite{Wu21AdvTforms}) attack uses a
neural network to create adversarial perturbations robust against
transformations for enhanced transferability, and achieves competitive 
transferability rates. However, unfortunately, we were unable to find a
publicly available implementation of the attack.
\cite{huang2019enhancing}'s
intermediate level attack improve \AE{} transferability by reducing the
variance of intermediate activations. We used the official 
implementation\footnote{\url{https://github.com/CUAI/Intermediate-Level-Attack}}
to test the attack on \cifarten{} with $\epsilon$=0.02 
and the VGG or DenseNet models as surrogates. The results showed
that the transferability rates were much less competitive that the three
baselines we considered (50.34\% vs.\ $>$54.00\% average transferability 
with a VGG surrogate, and 45.68\% vs.\ $>$56.56\% average transferability 
with a DenseNet surrogate). Therefore, we removed the intermediate level
attack for the remaining experiments.



==> app-parallel-composition.tex <==
\section{Parallel Composition v.s. Serial Composition}
\label{app:parcom}
%
%


==> app-proofs.tex <==
\section{Proofs} %
\label{app:proofs}


\label{app:proofs:theoA}


\parheading{Proof of \theoremref{theoA}}
  Augmenting $f$ with Gaussian noise, drawn from $\mathcal{N}(0, E)$,
  results in the so-called Weierstrass transform of $f$~\cite{salman2019provably}:
  
\centerline{\resizebox{\columnwidth}{!}{
$\begin{gathered}
\hat{f}(x)=(f * \mathcal{N}(0, E))(x) 
=\frac{1}{(2 \pi)^{n / 2}}  \int_{{R}^n} f(t) \exp \left(-\frac{1}{2}\|x-t\|^2\right) d t \\
=\int_{{R}^n} f(t) \frac{1}{(2 \pi)^{n / 2}} \exp \left(-\frac{1}{2}\|x-t\|^2\right) d t 
=\int_{{R}^n} \nabla_x\left(J\left(t, y, \theta\right)\right) \frac{1}{(2 \pi)^{n / 2}} \exp \left(-\frac{1}{2}\|x-t\|^2\right) d t
\end{gathered}$
}}
where $t$ is obtained after adding noise to $x$.
  
It suffices to show %
$u\cdot \nabla \hat{f}(x)\le I\cdot\sqrt{\frac{2}{\pi}}$.
holds for any unit vector $u$.
Note that:

\centerline{\resizebox{0.6\columnwidth}{!}{
$\begin{gathered}
\nabla \hat{f}(x)  =
\frac{1}{(2 \pi)^{n / 2}} \int_{{R}^n} f(t)(x-t)
\exp \left(-\frac{1}{2}\|x-t\|^2\right) d t
\end{gathered}$.
}}    
{\noindent Thus, using $|f(t)|\le I$, we get:}

\centerline{\resizebox{0.63\columnwidth}{!}{
$\begin{gathered}
u \!\cdot\! \nabla \hat{f}(x) \!\leq \! \frac{1}{(2 \pi)^{n / 2}}\! \int_{{R}^n} \! \!\!\!
\mid \! \! I  \! \cdot  \! u \! \cdot\! (x-t) \mid \exp \left(-\frac{1}{2}\|x-t\|^2\right) d t \\
 =\frac{I}{\sqrt{2 \pi}} \int_{-\infty}^{+\infty}|s| \exp \left(-\frac{1}{2} s^2\right) d s=I\cdot\sqrt{\frac{2}{\pi}} .
\end{gathered}$
}}


\label{app:proofs:theoB}


\parheading{Proof of \theoremref{theoB}}
It suffices to show %
$u\cdot \nabla \hat{f}(x)\le I\cdot\frac{\sqrt{2}}{\sqrt{\pi}*{\sigma}^2}$
holds for any unit vector $u$.
Note that:

\centerline{\resizebox{\columnwidth}{!}{
$\begin{gathered}
\hat{f}(x)=\left(f * \mathcal{N}\left(0, \sigma^2\right)\right)(x)
=\frac{1}{(2 \pi)^{n / 2} * \sigma} \int_{R^n} f(t) \exp \left(-\frac{1}{2}\|x-t\|^2 / \sigma^2\right) d t \\
=\int_{R^n} f(t) \frac{1}{(2 \pi)^{n / 2} / \sigma} \exp \left(-\frac{1}{2}\|x-t\|^2 / \sigma^2\right) d t
=\int_{R^n} \nabla_x(J(t, y, \theta)) \frac{1}{(2 \pi)^{n / 2} * \sigma} \exp \left(-\frac{1}{2}\|x-t\|^2 / \sigma^2\right) d t \\
\end{gathered}$
}}
Thus, if we compute the derivative of $\hat{f}(x)$, we would get:

\centerline{\resizebox{0.7\columnwidth}{!}{
$\begin{gathered}
\nabla \hat{f}(x)=
\frac{1}{(2 \pi)^{n / 2} * \sigma^3} \int_{R^n} f(t)(x-t) \exp \left(-\frac{1}{2}\|x-t\|^2 / \sigma^2\right) d t
\end{gathered}$
}}
{\noindent Now, using $|f(t)|\le I$, we get:}

\centerline{\resizebox{\columnwidth}{!}{
$
\begin{gathered}
u \cdot \nabla \hat{f}(x) \leq \frac{1}{(2 \pi)^{n / 2} * \sigma^3} \int_{R^n} \!\! |I \cdot u \cdot(x-t)| \exp \left(-\frac{1}{2}\|x-t\|^2 / \sigma^2\right) \! d t \\
=\frac{I}{\sqrt{2 \pi} * \sigma^3} \int_{-\infty}^{+\infty}|s| \exp \left(-\frac{1}{2} s^2 / \sigma^2\right) d s
=\frac{2 I}{\sqrt{2 \pi} * \sigma^3} \int_0^{+\infty} s \exp \left(-\frac{1}{2} s^2 / \sigma^2\right) d s \\
=\frac{2 I}{\sqrt{2 \pi} * \sigma^3} \int_0^{+\infty} \frac{1}{2} \exp \left(-\frac{1}{2} s^2 / \sigma^2\right) d s^2
=\frac{2 I}{\sqrt{2 \pi} * \sigma^3} \int_0^{+\infty} \frac{1}{2} \exp \left(-\frac{1}{2} x / \sigma^2\right) d x \quad\left(x=s^2\right) \\
=\left.\frac{2 I}{\sqrt{2 \pi} * \sigma^3} *\left(-\sigma * \exp \left(-\frac{1}{2} x / \sigma^2\right)\right)\right|_0 ^{\infty}
=I\cdot\frac{\sqrt{2}}{\sqrt{\pi}*{\sigma}^2}.
\end{gathered}
$
}}

\label{app:proofs:theoC}


\parheading{Proof of \theoremref{theoC}}
Again, it suffices to show
$u \cdot \nabla \hat{f}(x) \leq I \cdot A.$
holds for any unit-norm vector $u$. Note that:

\centerline{\resizebox{0.4\columnwidth}{!}{
$\begin{gathered}
  \hat{f}(x)=f * g(x)=\int_{{R}^n} f(t) g(t-x) d t
\end{gathered}$
}}

{\noindent Thus:}

\centerline{\resizebox{\columnwidth}{!}{
$
\begin{gathered}
u \cdot \nabla \hat{f}(x) =\int_{{R}^n}  f(t) \cdot u \cdot \nabla_t g(t-x) d t
\leq|\int_{{R}^n}  f(t) \cdot u \cdot \nabla_t g(t-x) d t|
\leq\int_{{R}^n} | f(t) \cdot u| \cdot |\nabla_t g(t-x) |d t\\
\leq \int_{{R}^n} I\cdot |\nabla_t g(t-x) |d t
\leq I |\int_{{R}^n} \nabla_x g(t-x) d t|=I \cdot A
\end{gathered}
$
}}




==> app-refined_admix.tex <==
\section{Refined admix augmentation}
Here we try to show our composition of various augmentations can help improve the transferability even though we do not alter  the augmentation. Take admix as an example. We compare performance of our  methodology and that method mentioned in the original paper\cite{Wang21Admix}.
\begin{table*}[!htbp]
\scriptsize
\centering
\caption{\label{tab:table-ref}This figure illustrates the transferability rate(\%) crafted by Inception-V3. The refined  \ASDTM{}represents our   composition method when including admix .}
\begin{tabular}{lllllll}
\toprule
 \textbf{Attack}& \textbf{Inc-v3}& \textbf{Inc-v4}&\textbf{Res-50}&\textbf{ Res-101}&\textbf{res-152}&\textbf{IncRes-v2}\\ \midrule
\ASDTM{} & {99.5} &92.3&88.5&87.0&85.3&90.9\\
  \SDTM{}&{100.0}&92.9&89.5&87.2&86.4&91.2\\
 refined-\ASDTM{}&100.0&94.7&91.9&90.3&88.7&93.3\\


 \midrule
\bottomrule
\end{tabular}


\end{table*}


==> app-time.tex <==
\section{Attack Run-Times}
\label{app:time}

\begin{table*}[t!]
\setlength\tabcolsep{3pt}
\small
\centering
\caption{\label{tab:timing}The number of samples augmented and the
  avg.\ time of crafting an \AE{} %
  per attack. Times were measured on an Nvidia A5000 GPU,
  on \imagenet{}, when attacking an
  Inc-v3, and averaged for 1K samples. For best
  transferability rates, \undp{} (marked with 
  \textsuperscript{(*)}) was run
  for 100 iterations, while other attacks were run for 10.
}
\centerline{ %
\begin{tabular}{l | r r r r | r r r r}
  \toprule
  \textbf{Attack} & \textbf{\ASDTM{}} & \textbf{\SDTM{}} &
  \textbf{\sdtv{}} & \textbf{\undp{}} & \textbf{\gsdt} &
  \textbf{\bestcombo} & \textbf{\subsetattack{30}} & \textbf{\advancedultimatecombo{}} \\ \midrule
  \textbf{Augmented samples} & 15 & 5 & 105 & 1 & 10 & 30 & 30 & 165 \\
  \textbf{Time (s)} & 1.68 & \textbf{0.72} & 11.29 & 1.65 & \textit{1.10} &
  3.62 & 5.54 & 40.27 \\ 

  

  \bottomrule
\end{tabular}} %

\end{table*}


==> app-upper-bound.tex <==
\section{Comparison with \bound{}}
\label{app:maxtransfer}

We used the Inc-v3 as surrogate model and 11 different attack
methods (namely, PI-FGSM~\cite{gao2020patch},
DI-\mifgsm~\cite{xie2019improving}, SI-NI-FGSM~\cite{lin2019nesterov},
\mifgsm{}, \admix{}-D-\mifgsm{}, \ASDTM{}, \gsdt{}, \ifgsm{}, \dt{},
\sdtv{}, \dst{}) to craft 11 adversarial examples for each
image in the \imagenet{} dataset. Subsequently, we measured how many
of the remaining \imagenet{} models are fooled for each of the 11
adversarial examples and selected the sample with the highest
transferability rates. We name the resulting attack
\bound{}. \tabref{tab:bound} compares \bound{}'s transferability rates
with the three baselines and \bestcombo{}.

\begin{table*}[!htbp]
\scriptsize
\centering
\caption{\label{tab:bound}The transferability rates (\%) of \bound{},
  \bestcombo{}, and the baselines, from Inc-v3 to other target models on the \imagenet{} dataset.}
\begin{tabular}{l | rrrrrrrrrr| r}
\toprule
 \textbf{Attack}& \textbf{Inc-v3}& \textbf{Inc-v4}&\textbf{Res-50}&\textbf{Res-101}&\textbf{Res-152}&\textbf{IncRes-v2} &  \textbf{Inc-v3$_{adv}$}& \textbf{Inc-v3$_{ens3}$}&\textbf{Inc-v3$_{ens4}$}&\textbf{ IncRes-v2$_{ens}$}&\textbf{ Avg.}\\ \midrule
 \ASDTM{} & \textit{99.5} &92.3&88.5&87.0&85.3&90.9&84.6&84.3&83.5&70.8&85.2\\
 \SDTM{}&\textbf{100.0}&92.9&89.5&87.2&86.4&91.2&81.3&81.2&77.7&61.4&83.2\\
 \sdtv{}&\textbf{100.0}&94.7&90.7&88.9&89.1&92.6&84.4&84.8&82.9&69.2&86.4\\
 \bound{} & \textbf{100.0} &\textit{96.9}&\textit{94.3}&\textit{93.9}&\textit{92.2}&\textit{95.7}&\textit{88.4}&\textit{90.0}&\textit{87.8}&\textit{77.5}&\textit{90.7}\\
 \bestcombo{} &\textbf{100.0}&\textit{98.0}&\textit{95.1}&\textit{94.3}&\textit{92.7}&\textit{97.1}&\textit{88.2}&\textit{88.7}&\textit{86.7}&\textit{72.6} &\textit{90.3}\\

  \advancedultimatecombo{} &\textbf{100.0}&\textbf{99.7}&\textbf{97.1}&\textbf{97.1}&\textbf{96.1}&\textbf{98.8}&\textbf{95.7}&\textbf{96.2}&\textbf{95.3}&\textbf{87.7} &\textbf{96.0}\\



  


 \midrule
\bottomrule
\end{tabular}


\end{table*}


==> figures/single_attack_result.tex <==














































 


























































































 











  














==> tables/genetic-overhead.tex <==
\begin{table*}[t!]
\small
\centering
\caption{\label{tab:genetic-overhead}
  The ratio (\%) between the total number of augmentation combinations
  tested by genetic search and the entire search space ($2^7$) for
  a varied number of $n_\mathit{gen}$ search iterations (rows) and
  population sizes (columns).
  The Inc-v3 model was used as a surrogate, while the remaining nine
  \imagenet{} models served as targets.
  The reported ratios are averaged over 100 runs of genetic search.} 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{l|rrrrrrrrrrrrr}
\toprule
 &     2 &     4 &     6 &     8 &    10 &    12 &    14 &    16 &    18 &    20 &    22 &    24 &    26 \\
\midrule
    10 & 10.23 & 12.48 & 14.43 & 16.39 & 16.67 & 18.47 & 18.85 & 19.60 & 20.88 & 20.28 & 21.54 & 22.84 & 23.19 \\
    20 & 19.42 & 24.31 & 28.20 & 30.22 & 31.95 & 34.31 & 34.84 & 36.25 & 36.15 & 37.91 & 37.98 & 40.16 & 39.53 \\
    30 & 26.67 & 33.55 & 38.84 & 41.19 & 43.51 & 44.14 & 46.82 & 47.62 & 48.80 & 49.98 & 51.05 & 52.14 & 52.21 \\
    40 & 33.32 & 41.56 & 46.10 & 49.27 & 52.17 & 53.65 & 54.75 & 56.05 & 57.70 & 57.96 & 59.21 & 60.50 & 59.79 \\
    50 & 39.54 & 47.97 & 53.47 & 55.33 & 58.09 & 59.24 & 60.98 & 62.55 & 63.29 & 63.56 & 65.77 & 65.59 & 66.59 \\
    60 & 44.70 & 53.44 & 58.60 & 61.31 & 62.15 & 64.66 & 65.62 & 67.28 & 67.49 & 68.75 & 69.30 & 69.68 & 71.05 \\
    70 & 48.80 & 58.05 & 62.50 & 65.46 & 67.79 & 68.42 & 69.93 & 70.59 & 71.52 & 72.35 & 73.62 & 73.58 & 74.79 \\
    80 & 52.86 & 61.74 & 66.20 & 68.98 & 69.95 & 71.72 & 72.17 & 73.26 & 74.69 & 74.43 & 75.91 & 76.50 & 77.67 \\
    90 & 57.08 & 65.18 & 69.42 & 71.05 & 73.48 & 73.88 & 75.29 & 75.93 & 76.83 & 78.41 & 78.21 & 79.06 & 79.27 \\
   100 & 60.14 & 67.47 & 71.84 & 73.95 & 75.38 & 76.96 & 77.52 & 78.07 & 79.63 & 79.64 & 80.45 & 80.57 & 81.94 \\
   110 & 63.16 & 70.88 & 74.24 & 75.95 & 77.54 & 78.69 & 79.52 & 79.99 & 81.24 & 81.39 & 82.24 & 82.19 & 83.39 \\
   120 & 65.95 & 73.34 & 76.41 & 78.02 & 79.28 & 80.34 & 81.10 & 81.85 & 82.61 & 83.01 & 83.68 & 84.49 & 84.80 \\
   130 & 68.38 & 74.66 & 78.12 & 79.84 & 80.49 & 81.84 & 82.23 & 83.02 & 84.16 & 84.10 & 84.61 & 85.74 & 85.83 \\
   140 & 69.73 & 76.53 & 79.77 & 81.30 & 81.86 & 82.57 & 83.57 & 84.71 & 84.96 & 85.82 & 85.89 & 86.77 & 87.07 \\
   150 & 72.16 & 78.66 & 80.71 & 82.16 & 84.49 & 84.19 & 85.05 & 85.98 & 86.59 & 87.27 & 86.65 & 87.59 & 87.64 \\
\bottomrule
\end{tabular}}


\end{table*}


==> tables/genetic-result.tex <==
\begin{table*}[t!]
\small
\centering
\caption{\label{tab:genetic-result}The ratio (\%) between average
  transferability rates of the best performing augmentation combination
  found by genetic search compared to \bestcombo{}, for
  a varied number of $n_\mathit{gen}$ search iterations (rows) and
  population sizes (columns).
  The Inc-v3 model was used as a surrogate, while the remaining nine
  \imagenet{} models served as targets.
  The reported ratios are averaged over 100 runs of genetic search.}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{l|rrrrrrrrrrrrr}
\toprule
  &     2 &     4 &     6 &     8 &    10 &    12 &    14 &    16 &    18 &    20 &    22 &    24 &    26 \\
\midrule
    10 & 98.99 & 98.46 & 97.81 & 98.40 & 98.37 & 97.92 & 98.07 & 98.55 & 98.20 & 98.10 & 97.89 & 98.24 & 98.12 \\
    20 & 99.41 & 99.31 & 99.32 & 99.38 & 99.30 & 99.35 & 99.20 & 99.11 & 99.30 & 99.02 & 99.20 & 99.14 & 99.03 \\
    30 & 99.70 & 99.67 & 99.59 & 99.55 & 99.59 & 99.53 & 99.48 & 99.57 & 99.42 & 99.56 & 99.55 & 99.40 & 99.59 \\
    40 & 99.78 & 99.67 & 99.72 & 99.71 & 99.70 & 99.71 & 99.62 & 99.68 & 99.66 & 99.76 & 99.71 & 99.70 & 99.68 \\
    50 & 99.87 & 99.83 & 99.83 & 99.80 & 99.86 & 99.82 & 99.82 & 99.82 & 99.79 & 99.79 & 99.77 & 99.82 & 99.77 \\
    60 & 99.88 & 99.90 & 99.90 & 99.88 & 99.89 & 99.84 & 99.84 & 99.89 & 99.81 & 99.86 & 99.83 & 99.85 & 99.88 \\
    70 & 99.90 & 99.88 & 99.91 & 99.92 & 99.89 & 99.90 & 99.90 & 99.89 & 99.86 & 99.88 & 99.87 & 99.92 & 99.91 \\
    80 & 99.93 & 99.93 & 99.94 & 99.91 & 99.92 & 99.93 & 99.94 & 99.90 & 99.92 & 99.95 & 99.92 & 99.93 & 99.92 \\
    90 & 99.94 & 99.94 & 99.92 & 99.94 & 99.96 & 99.97 & 99.93 & 99.94 & 99.95 & 99.96 & 99.95 & 99.95 & 99.96 \\
   100 & 99.96 & 99.95 & 99.95 & 99.97 & 99.94 & 99.95 & 99.92 & 99.93 & 99.95 & 99.95 & 99.95 & 99.97 & 99.96 \\
   110 & 99.95 & 99.96 & 99.95 & 99.96 & 99.97 & 99.96 & 99.95 & 99.97 & 99.96 & 99.98 & 99.97 & 99.97 & 99.96 \\
   120 & 99.97 & 99.97 & 99.97 & 99.96 & 99.97 & 99.97 & 99.97 & 99.96 & 99.98 & 99.98 & 99.97 & 99.96 & 99.98 \\
   130 & 99.98 & 99.96 & 99.97 & 99.97 & 99.97 & 99.99 & 99.98 & 99.96 & 99.97 & 99.97 & 99.98 & 99.97 & 99.99 \\
   140 & 99.97 & 99.98 & 99.98 & 99.98 & 99.99 & 99.97 & 99.98 & 99.98 & 99.99 & 99.97 & 99.99 & 99.98 & 99.99 \\
   150 & 99.98 & 99.99 & 99.99 & 99.97 & 99.98 & 99.99 & 99.99 & 99.98 & 99.99 & 99.97 & 99.99 & 99.99 & 99.97 \\
\bottomrule
\end{tabular}}

\end{table*}

